PROflow: An iterative refinement model for PROTAC-induced structure prediction

Proteolysis targeting chimeras (PROTACs) are small molecules that trigger the breakdown of traditionally ``undruggable'' proteins by binding simultaneously to their targets and degradation-associated proteins. A key challenge in their rational design is understanding their structural basis of activity. Due to the lack of crystal structures (18 in the PDB), existing PROTAC docking methods have been forced to simplify the problem into a distance-constrained protein-protein docking task. To address the data issue, we develop a novel pseudo-data generation scheme that requires only binary protein-protein complexes. This new dataset enables PROflow, an iterative refinement model for PROTAC-induced structure prediction that models the full PROTAC flexibility during constrained protein-protein docking. PROflow outperforms the state-of-the-art across docking metrics and runtime. Its inference speed enables the large-scale screening of PROTAC designs, and computed properties of predicted structures achieve statistically significant correlations with published degradation activities.

==> tables/Tab_real.tex <==
\begin{table*}[t]
\begin{small}\begin{center}
\setlength\tabcolsep{3 pt}
% \renewcommand\arraystretch{1.2}
\caption{\textbf{Realistic docking results (apo structures).} Methods marked $^*$ did not consider the PROTAC at all. The best-performing method is emphasized in bold. None of the methods utilize re-ranking or clustering for prediction selection.}
\label{tab:real}
\vskip 0.15in
\begin{tabular}{l ccc ccc cc}
\toprule
& \multicolumn{3}{c}{Complex RMSD (\textup{\AA})}
& \multicolumn{3}{c}{Interface RMSD (\textup{\AA})}
& \multicolumn{2}{c}{Fnat}
\\
\cmidrule(l{\tabcolsep}){2-4}
\cmidrule(l{\tabcolsep}){5-7}
\cmidrule(l{\tabcolsep}){8-9}
Model & Mean $\downarrow$ & Median $\downarrow$
& $<$20~$\uparrow$  & Mean $\downarrow$
& Median $\downarrow$
& $<$10~$\uparrow$  &Mean $\uparrow$  &  Median $\uparrow$
\\ \midrule
Alphafold Multimer$^*$
& 12.94 & 12.52 & 0.865 & 9.80 & 9.15 & 0.563 & 0.208 & \textbf{0.200}
\\
DiffDock-PP$^*$
& 21.45 & 21.39 & 0.380 & 12.65 & 10.97 & 0.446 &0.206 &0.079
\\
PROTACability
& 27.58 & 27.48 &  0.641
& 25.67 & 25.23 & 0.275 & 0.118 & 0.080 \\
PRossetaC
& 15.33 & 15.49 & 0.856 & 12.13 & 12.20 & 0.367 &0.095 & 0.071 \\ \midrule
PROflow
& \textbf{12.16}
& \textbf{12.45}
& \textbf{0.995} & \textbf{8.35} & \textbf{8.62} & \textbf{0.643} & \textbf{0.236} & 0.188 \\
\bottomrule
\end{tabular}
\end{center}\end{small}
\vskip -0.1in
\end{table*}


==> tables/Tab_redock.tex <==
\begin{table*}[t]
\begin{small}\begin{center}
% \renewcommand\arraystretch{1.2}
\setlength\tabcolsep{3 pt}
\caption{\textbf{Re-docking results (holo structures).} Methods marked $^*$ did not consider the PROTAC at all. Runtimes marked $\dagger$ were performed exclusively on CPU (method does not support GPU). The best-performing method is emphasized in bold. None of the methods utilize re-ranking or clustering for prediction selection.}
\label{tab:redock}
\vskip 0.15in
\begin{tabular}{l ccc ccc cc r}
\toprule
& \multicolumn{3}{c}{Complex RMSD (\textup{\AA})}
& \multicolumn{3}{c}{Interface RMSD (\textup{\AA})}
& \multicolumn{2}{c}{Fnat}
& Runtime (s)
\\
\cmidrule(l{\tabcolsep}){2-4}
\cmidrule(l{\tabcolsep}){5-7}
\cmidrule(l{\tabcolsep}){8-9}
\cmidrule(l{\tabcolsep}){10-10}
Model & Mean $\downarrow$ & Median $\downarrow$
& $<$20~$\uparrow$  & Mean $\downarrow$
& Median $\downarrow$
& $<$10~$\uparrow$  &Mean $\uparrow$  &  Median $\uparrow$
& Mean $\downarrow$
\\ \midrule
AF-Multimer$^*$ 
& 14.83 & 15.44 & 0.812 & 10.49 & 10.81 & 0.539 & 0.221 & 0.203 & 735$\dagger$ 
\\
DiffDock-PP$^*$ 
& 19.67 & 19.66 & 0.510 & 10.04 & 10.14 & 0.509 &0.229 &0.199 
& 150 
\\
PROTACability 
& \textbf{12.45} & \textbf{12.26} &  0.926 
& 11.21 & 10.79 & 0.496 & 0.144 & 0.050 & 144$\dagger$ 
\\
PRossetaC 
& 13.06 & 13.37 & 0.954 & 10.03 & 10.12 & 0.487 &0.114 & 0.085 & 3015$\dagger$ 
\\ \midrule
PROflow 
& 12.85 & 13.12 & \textbf{0.975} & \textbf{8.20} & \textbf{8.16} & \textbf{0.740} & \textbf{0.264} & \textbf{0.211} & \textbf{44} 
\\ \midrule
\end{tabular}
\end{center}\end{small}
\vskip -0.1in
\end{table*}


==> tables/testset_pdbid.tex <==
\begin{table}[]
\begin{tabular}{cc}
\hline
         & PDB ID                                                                         \\ \hline
Test set & 5T35, 6BN\&, 6BOY, 6HAX, 7PI4, 6HR2, 6W\&O, 6W8I, 6ZHC, 7JTO, 7JTP, 7KHH, 7Q2J \\ \hline
\end{tabular}
\end{table}

==> tex/0-abstract_old.tex <==
\begin{abstract}
%Proteolysis targeting chimeras (PROTACs) are next generation therapeutics capable of degrading traditionally ``undruggable'' proteins, but a significant hurdle in their rational design is the lack of structural data.
Proteolysis targeting chimeras (PROTACs) are small molecules that induce proximity between the protein of interest (POI) and an E3 ligase, which shows great potential in degrading traditionally “undruggable” proteins.
%Contrary to small molecule drugs that bind directly to their protein targets, PROTACs induce proximity between the protein of interest and an E3 ubiquitin ligase, which triggers the cell's innate protein degradation pathways.
%Modeling the subsequent ternary complex is crucial to understanding this interaction.
Predicting the PORTAC-induced ternary structure is crucial for designing novel PROTACS and comprehending the machenism of existing drugs.
%However, combining existing methods for protein-small molecule or protein-protein docking is insufficient in this regime, where the PROTAC itself is highly flexible, and the protein-protein interactions are low affinity.
However, it requires modeling highly flexible conformation of PROTACs as well as the binding pose of E3 ligase to the POI simultaneously. Applying machine learning models to ternary structure docking is challenging because of the complexity of sampling with multiple degrees of freedom in the three-body system and the lack of data. 
In this work, we initially introduce a definition of the product space for docking, aiming to minimize redundant degrees of freedom. Subsequently, we propose a flow-matching model on it named PROflow, which effectively captures the relative positions of proteins distributed across chemically plausible PROTAC conformations. By jointly modeling the relative positions of protein-protein and protein-ligand, our method resolves conflicts involving ligands and proteins shifting from each others' energetically favorable conformations. In addition, an innovative pseudo-data generation method is designed so that the model could be trained on large numbers of protein-protein complexes. Empirically validating PROflow, we successfully predict experimentally-solved ternary structures, achieving favorable interface-RMSD and faster inference times.
%In this work, we propose PROflow, a flow-matching model that jointly models the relative positions of both proteins and the distribution over chemically-plausible PROTAC conformations, while only requiring binary data to train.
%Empirically, our model significantly outperforms the state-of-the-art (\#\#) while offering faster inference times.
\end{abstract}
